Stochastic Configuration Machines for Industrial Artificial Intelligence

Real-time predictive modelling with desired accuracy is highly expected in industrial artificial intelligence (IAI), where neural networks play a key role. Neural networks in IAI require powerful, high-performance computing devices to operate a large number of floating point data. Based on stochastic configuration networks (SCNs), this paper proposes a new randomized learner model, termed stochastic configuration machines (SCMs), to stress effective modelling and data size saving that are useful and valuable for industrial applications. Compared to SCNs and random vector functional-link (RVFL) nets with binarized implementation, the model storage of SCMs can be significantly compressed while retaining favourable prediction performance. Besides the architecture of the SCM learner model and its learning algorithm, as an important part of this contribution, we also provide a theoretical basis on the learning capacity of SCMs by analysing the model's complexity. Experimental studies are carried out over some benchmark datasets and three industrial applications. The results demonstrate that SCM has great potential for dealing with industrial data analytics.

==> tables/SCM_Candidates.tex <==
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{c|ccc}
    \hline
    Data Set & Sum (min(ksim) > 0) & Sum (min(ksim) $<=$ 0) & Percent \bigstrut[b]\\
    \hline
    \hline
    R-DB1 & TODO & TODO & 0.00\% \bigstrut[t]\\
    R-DB2 & 5093 & 230907 & 2.21\% \\
    R-DB3 & TODO & TODO & 0.00\% \\
    R-DB4 & TODO & TODO & 0.00\% \\
    R-DB5 & TODO & TODO & 0.00\% \\
    R-DB6 & TODO & TODO & 0.00\% \\
    R-DB7 & TODO & TODO & 0.00\% \\
    R-DB8 & TODO & TODO & 0.00\% \\
    R-DB9 & TODO & TODO & 0.00\% \\
    R-DB10 & 49790 & 4120210 & 1.21\% \\
    C-DB1 & TODO & TODO & 0.00\% \\
    C-DB2 & TODO & TODO & 0.00\% \\
    C-DB3 & TODO & TODO & 0.00\% \\
    C-DB4 & 7109 & 672891 & 1.06\% \\
    C-DB5 & 37443 & 7880557 & 0.48\% \bigstrut[b]\\
    \hline
    \end{tabular}%
  \label{tab:SCM_Candidates}%
\end{table}%
